Resilient expansion planning of virtual energy plant with an integrated energy system -- reliability criteria of lines and towers

Virtual power plants, while being virtual, rely on a physical network for operations. The portfolio of the virtual power plants is flexible in facilitating a wide range of resources including the local heat pumps. The power transmission network has the responsibility to ensure the security of supply, reliability of operation, planning, and expansion. The power transmission network and apparatus including lines and towers are also aging with time. Furthermore, the transmission network covers a large geographical area which is expensive to maintain. The objective of this paper is to investigate the effect of power network conditions on power network expansion planning. The condition of the power network is determined by the maintenance cost of lines and a health index and a risk factor associated with the tower. The investigation begins with answering how the inclusion of heat pump impacts the decisions on network interventions. Thereafter, the condition network is factored into the decision-making by better understanding the impact of the network condition on the overall expansion planning. Furthermore, many sensitivity analyses are conducted to evaluate the trade-offs between decision variables such as cost of heat pump, coefficient of performance of heat pump, risk factors, and line and tower costs.

==> sec/04_sec.tex <==
\hl{Sambeet and Chiara co-lead}

\subsection{trade offs}

\subsubsection{COP vs network reconfig}

\subsubsection{HP cost vs COP}


\subsection{Heat demand vs costs}


\subsubsection{Maintenance cost vs network reconfig}

\subsubsection{learning effect}


\subsection{Network Tower and lines}


\subsection{Network health and risk}

\subsubsection{Network length}

